PGSR: Planar-based Gaussian Splatting for Efficient and High-Fidelity Surface Reconstruction

Recently, 3D Gaussian Splatting (3DGS) has attracted widespread attention due to its high-quality rendering, and ultra-fast training and rendering speed. However, due to the unstructured and irregular nature of Gaussian point clouds, it is difficult to guarantee geometric reconstruction accuracy and multi-view consistency simply by relying on image reconstruction loss. Although many studies on surface reconstruction based on 3DGS have emerged recently, the quality of their meshes is generally unsatisfactory. To address this problem, we propose a fast planar-based Gaussian splatting reconstruction representation (PGSR) to achieve high-fidelity surface reconstruction while ensuring high-quality rendering. Specifically, we first introduce an unbiased depth rendering method, which directly renders the distance from the camera origin to the Gaussian plane and the corresponding normal map based on the Gaussian distribution of the point cloud, and divides the two to obtain the unbiased depth. We then introduce single-view geometric, multi-view photometric, and geometric regularization to preserve global geometric accuracy. We also propose a camera exposure compensation model to cope with scenes with large illumination variations. Experiments on indoor and outdoor scenes show that our method achieves fast training and rendering while maintaining high-fidelity rendering and geometric reconstruction, outperforming 3DGS-based and NeRF-based methods.

==> reference.tex <==
\begin{thebibliography}{1}
\bibliographystyle{IEEEtran}

\bibitem{deng2022fov}
Nianchen Deng, Zhenyi He, Jiannan Ye, Budmonde Duinkharjav, Praneeth Chakravarthula, Xubo Yang, and Qi~Sun.
\newblock {Fov-NeRF: Foveated} neural radiance fields for virtual reality.
\newblock {\em IEEE Transactions on Visualization and Computer Graphics}, 28(11):3854--3864, 2022.

\bibitem{ye2021superplane}
Weicai Ye, Hai Li, Tianxiang Zhang, Xiaowei Zhou, Hujun Bao, Guofeng Zhang.
\newblock SuperPlane: 3D plane detection and description from a single image.
\newblock In {\em IEEE Virtual Reality and 3D User Interfaces}, 207--215, 2021.

\bibitem{poole2022dreamfusion}
Ben Poole, Ajay Jain, Jonathan~T Barron, and Ben Mildenhall.
\newblock Dreamfusion: Text-to-3d using 2d diffusion.
\newblock {\em arXiv preprint arXiv:2209.14988}, 2022.

\bibitem{tang2023dreamgaussian}
Jiaxiang Tang, Jiawei Ren, Hang Zhou, Ziwei Liu, and Gang Zeng.
\newblock Dreamgaussian: Generative gaussian splatting for efficient 3d content creation.
\newblock {\em arXiv preprint arXiv:2309.16653}, 2023.

\bibitem{gao2024luminat2x}
Peng Gao, Le Zhuo, Dongyang Liu, Ruoyi Du, Xu Luo, Longtian Qiu, Yuhang Zhang, Rongjie Huang, Shijie Geng, Renrui Zhang, unlin Xie, Wenqi Shao, Zhengkai Jiang, Tianshuo Yang, Weicai Ye, Tong He, Jingwen He, Yu Qiao, Hongsheng Li.
\newblock Lumina-T2X: Transforming Text into Any Modality, Resolution, and Duration via Flow-based Large Diffusion Transformers.
\newblock {\em arxiv preprint arXiv:2405.05945}, 2024.

% \bibitem{ye2024DiffPano}
% Weicai Ye, Chenhao Ji, Zheng Chen, Junyao Gao, Xiaoshui Huang, Song-Hai Zhang, Wanli Ouyang, Tong He, Cairong Zhao, Guofeng Zhang.
% \newblock DiffPano: Scalable and Consistent Text to Panorama Generation with Spherical Epipolar-Aware Diffusion.
% \newblock {\em arxiv preprint}, 2024.

\bibitem{chen2024AM}
Yiwen Chen, Tong He, Di Huang, Weicai Ye, Sijin Chen, Jiaxiang Tang, Zhongang Cai, Lei Yang, Gang Yu, Guosheng Lin, Chi Zhang.
\newblock Artist-Created Mesh Generation with Autoregressive Transformers.
\newblock {\em arxiv preprint}, 2024.

\bibitem{li2020saliency}
Hai Li, Weicai Ye, Guofeng Zhang, Sanyuan Zhang, Hujun Bao.
\newblock Saliency guided subdivision for single-view mesh reconstruction.
\newblock In {\em International Conference on 3D Vision}, 1098--1107, 2020.

\bibitem{liu2021coxgraph}
Xiangyu Liu, Weicai Ye, Chaoran Tian, Zhaopeng Cui, Hujun Bao, Guofeng Zhang.
\newblock Coxgraph: multi-robot collaborative, globally consistent, online dense reconstruction system.
\newblock In {\em IEEE/RSJ International Conference on Intelligent Robots and Systems}, 8722--8728, 2021.

\bibitem{ye2023PVO}
Weicai Ye, Xinyue Lan, Shuo Chen, Yuhang Ming, Xingyuan Yu, Hujun Bao, Zhaopeng Cui, Guofeng Zhang.
\newblock PVO: Panoptic Visual Odometry.
\newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, 9579-9589, 2023.

\bibitem{ye2022deflowslam}
Weicai Ye, Xingyuan Yu, Xinyue Lan, Yuhang Ming, Jinyu Li, Hujun Bao, Zhaopeng Cui, Guofeng Zhang.
\newblock DeFlowSLAM: Self-Supervised Scene Motion Decomposition for Dynamic Dense SLAM.
\newblock {\em arXiv preprint arXiv:2207.08794}, 2022.

% \bibitem{ye2024DATAP-SfM}
% Weicai Ye, Xinyu Chen, Ruohao Zhan, Di Huang, Xiaoshui Huang, Haoyi Zhu, Hujun Bao, Wanli Ouyang, Tong He, Guofeng Zhang.
% \newblock DATAP-SfM: Dynamic-Aware Tracking Any Point for Structure from Motion in the Wild.
% \newblock {\em arXiv preprint}, 2022.

\bibitem{mildenhall2021nerf}
Ben Mildenhall, Pratul~P Srinivasan, Matthew Tancik, Jonathan~T Barron, Ravi Ramamoorthi, and Ren Ng.
\newblock NeRF: Representing scenes as neural radiance fields for view synthesis.
\newblock {\em Communications of the ACM}, 65(1):99--106, 2021.

\bibitem{Ye2023IntrinsicNeRF}
Weicai Ye, Shuo Chen, Chong Bao, Hujun Bao, Marc Pollefeys, Zhaopeng Cui, and Guofeng Zhang.
\newblock IntrinsicNeRF: Learning Intrinsic Neural Radiance Fields for Editable Novel View Synthesis.
\newblock In {\em Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 339--351, 2023.

\bibitem{huang2024nerfdet++}
Chenxi Huang, Yuenan Hou, Weicai Ye, Di Huang, Xiaoshui Huang, Binbin Lin, Deng Cai,  Wanli Ouyang.
\newblock NeRF-Det++: Incorporating Semantic Cues and Perspective-aware Depth Supervision for Indoor Multi-View 3D Detection.
\newblock {\em arXiv preprint arXiv:2402.14464}, 2024.

\bibitem{ming2022idf}
Yuhang Ming, Weicai Ye, Andrew Calway.
\newblock idf-SLAM: End-to-end rgb-d slam with neural implicit mapping and deep feature tracking.
\newblock {\em arXiv preprint arXiv:2209.07919}, 2022.


\bibitem{barron2021mip}
Jonathan~T Barron, Ben Mildenhall, Matthew Tancik, Peter Hedman, Ricardo Martin-Brualla, and Pratul~P Srinivasan.
\newblock Mip-NeRF: A multiscale representation for anti-aliasing neural radiance fields.
\newblock In {\em Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 5855--5864, 2021.

\bibitem{barron2023zip}
Jonathan~T Barron, Ben Mildenhall, Dor Verbin, Pratul~P Srinivasan, and Peter Hedman.
\newblock Zip-NeRF: Anti-aliased grid-based neural radiance fields.
\newblock In {\em Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 19697--19705, 2023.

\bibitem{muller2022instant}
Thomas M{\"u}ller, Alex Evans, Christoph Schied, and Alexander Keller.
\newblock Instant neural graphics primitives with a multiresolution hash encoding.
\newblock {\em ACM transactions on graphics (TOG)}, 41(4):1--15, 2022.

\bibitem{li2023neuralangelo}
Zhaoshuo Li, Thomas M{\"u}ller, Alex Evans, Russell~H Taylor, Mathias Unberath, Ming-Yu Liu, and Chen-Hsuan Lin.
\newblock Neuralangelo: High-fidelity neural surface reconstruction.
\newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 8456--8465, 2023.

\bibitem{wang2021neus}
Peng Wang, Lingjie Liu, Yuan Liu, Christian Theobalt, Taku Komura, and Wenping Wang.
\newblock NeuS: Learning neural implicit surfaces by volume rendering for multi-view reconstruction.
\newblock {\em arXiv preprint arXiv:2106.10689}, 2021.

\bibitem{kerbl20233d}
Bernhard Kerbl, Georgios Kopanas, Thomas Leimk{\"u}hler, and George Drettakis.
\newblock 3d gaussian splatting for real-time radiance field rendering.
\newblock {\em ACM Transactions on Graphics}, 42(4):1--14, 2023.

\bibitem{guedon2023sugar}
Antoine Gu{\'e}don and Vincent Lepetit.
\newblock SuGaR: Surface-aligned gaussian splatting for efficient 3d mesh reconstruction and high-quality mesh rendering.
\newblock {\em arXiv preprint arXiv:2311.12775}, 2023.

\bibitem{jiang2023gaussianshader}
Yingwenqi Jiang, Jiadong Tu, Yuan Liu, Xifeng Gao, Xiaoxiao Long, Wenping Wang, and Yuexin Ma.
\newblock Gaussianshader: 3d gaussian splatting with shading functions for reflective surfaces.
\newblock {\em arXiv preprint arXiv:2311.17977}, 2023.

\bibitem{jensen2014large}
Rasmus Jensen, Anders Dahl, George Vogiatzis, Engin Tola, and Henrik Aan{\ae}s.
\newblock Large scale multi-view stereopsis evaluation.
\newblock In {\em Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 406--413, 2014.

\bibitem{knapitsch2017tanks}
Arno Knapitsch, Jaesik Park, Qian-Yi Zhou, and Vladlen Koltun.
\newblock Tanks and temples: Benchmarking large-scale scene reconstruction.
\newblock {\em ACM Transactions on Graphics (ToG)}, 36(4):1--13, 2017.

\bibitem{campos2021orb}
Carlos Campos, Richard Elvira, Juan J~G{\'o}mez Rodr{\'\i}guez, Jos{\'e}~MM Montiel, and Juan~D Tard{\'o}s.
\newblock Orb-SLAM3: An accurate open-source library for visual, visual--inertial, and multimap SLAM.
\newblock {\em IEEE Transactions on Robotics}, 37(6):1874--1890, 2021.

\bibitem{chen2021rnin}
Danpeng Chen, Nan Wang, Runsen Xu, Weijian Xie, Hujun Bao, and Guofeng Zhang.
\newblock RNIN-VIO: Robust neural inertial navigation aided visual-inertial odometry in challenging scenes.
\newblock In {\em 2021 IEEE International Symposium on Mixed and Augmented Reality (ISMAR)}, pages 275--283. IEEE, 2021.

\bibitem{chen2022vip}
Danpeng Chen, Shuai Wang, Weijian Xie, Shangjin Zhai, Nan Wang, Hujun Bao, and Guofeng Zhang.
\newblock VIP-SLAM: An efficient tightly-coupled RGB-D visual inertial planar SLAM.
\newblock In {\em 2022 International Conference on Robotics and Automation (ICRA)}, pages 5615--5621. IEEE, 2022.

\bibitem{Moulon2012}
Pierre Moulon, Pascal Monasse, and Renaud Marlet.
\newblock Adaptive structure from motion with a~contrario model estimation.
\newblock In {\em Proceedings of the Asian Computer Vision Conference (ACCV 2012)}, pages 257--270. Springer Berlin Heidelberg, 2012.

\bibitem{schonberger2016structure}
Johannes~L Schonberger and Jan-Michael Frahm.
\newblock Structure-from-motion revisited.
\newblock In {\em Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 4104--4113, 2016.

\bibitem{wu2013towards}
Changchang Wu.
\newblock Towards linear-time incremental structure from motion.
\newblock In {\em 2013 International Conference on 3D Vision-3DV 2013}, pages 127--134. IEEE, 2013.

\bibitem{Accurate}
Yasutaka Furukawa and Jean Ponce.
\newblock Accurate, dense, and robust multiview stereopsis.
\newblock {\em IEEE Transactions on Pattern Analysis and Machine Intelligence}, 32(8):1362--1376, 2010.

\bibitem{lhuillier2005quasi}
Maxime Lhuillier and Long Quan.
\newblock A quasi-dense approach to surface reconstruction from uncalibrated images.
\newblock {\em IEEE transactions on pattern analysis and machine intelligence}, 27(3):418--433, 2005.

\bibitem{kutulakos2000theory}
Kiriakos~N Kutulakos and Steven~M Seitz.
\newblock A theory of shape by space carving.
\newblock {\em International journal of computer vision}, 38:199--218, 2000.

\bibitem{campbell2008using}
Neill~DF Campbell, George Vogiatzis, Carlos Hern{\'a}ndez, and Roberto Cipolla.
\newblock Using multiple hypotheses to improve depth-maps for multi-view stereo.
\newblock In {\em Computer Vision--ECCV 2008: 10th European Conference on Computer Vision, Marseille, France, October 12-18, 2008, Proceedings, Part I 10}, pages 766--779. Springer, 2008.

\bibitem{galliani2015massively}
Silvano Galliani, Katrin Lasinger, and Konrad Schindler.
\newblock Massively parallel multiview stereopsis by surface normal diffusion.
\newblock In {\em Proceedings of the IEEE international conference on computer vision}, pages 873--881, 2015.

\bibitem{schoenberger2016mvs}
Johannes~Lutz Sch\"{o}nberger, Enliang Zheng, Marc Pollefeys, and Jan-Michael Frahm.
\newblock Pixelwise view selection for unstructured multi-view stereo.
\newblock In {\em European Conference on Computer Vision (ECCV)}, 2016.

\bibitem{barnes2009patchmatch}
Connelly Barnes, Eli Shechtman, Adam Finkelstein, and Dan~B Goldman.
\newblock Patchmatch: A randomized correspondence algorithm for structural image editing.
\newblock {\em ACM Trans. Graph.}, 28(3):24, 2009.

\bibitem{cazals2006delaunay}
Fr{\'e}d{\'e}ric Cazals and Joachim Giesen.
\newblock Delaunay triangulation based surface reconstruction.
\newblock In {\em Effective computational geometry for curves and surfaces}, pages 231--276. Springer, 2006.

\bibitem{kazhdan2006poisson}
Michael Kazhdan, Matthew Bolitho, and Hugues Hoppe.
\newblock Poisson surface reconstruction.
\newblock In {\em Proceedings of the fourth Eurographics symposium on Geometry processing}, volume~7, 2006.

\bibitem{kazhdan2013screened}
Michael Kazhdan and Hugues Hoppe.
\newblock Screened poisson surface reconstruction.
\newblock {\em ACM Transactions on Graphics (ToG)}, 32(3):1--13, 2013.

\bibitem{sarlin2019coarse}
Paul-Edouard Sarlin, Cesar Cadena, Roland Siegwart, and Marcin Dymczyk.
\newblock From coarse to fine: Robust hierarchical localization at large scale.
\newblock In {\em CVPR}, 2019.

\bibitem{wang2021patchmatchnet}
Fangjinhua Wang, Silvano Galliani, Christoph Vogel, Pablo Speciale, and Marc Pollefeys.
\newblock Patchmatchnet: Learned multi-view patchmatch stereo.
\newblock In {\em Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 14194--14203, 2021.

\bibitem{Fan:2017:Point}
Haoqiang Fan, Hao Su, and Leonidas~J. Guibas.
\newblock A point set generation network for {3D} object reconstruction from a single image.
\newblock In {\em {IEEE} Conference on Computer Vision and Pattern Recognition}, pages 2463--2471, 2017.

\bibitem{Lin:2018:Learning}
Chen{-}Hsuan Lin, Chen Kong, and Simon Lucey.
\newblock Learning efficient point cloud generation for dense {3D} object reconstruction.
\newblock In {\em Conference on Artificial Intelligence}, pages 7114--7121, 2018.

\bibitem{Choy:2016:3d}
Christopher~B. Choy, Danfei Xu, JunYoung Gwak, Kevin Chen, and Silvio Savarese.
\newblock {3D-R2N2}: {A} unified approach for single and multi-view {3D} object reconstruction.
\newblock In {\em European Conference on Computer Vision}, volume 9912, pages 628--644, 2016.

\bibitem{Xie:2019:Pix2vox}
Haozhe Xie, Hongxun Yao, Xiaoshuai Sun, Shangchen Zhou, and Shengping Zhang.
\newblock Pix2{V}ox: Context-aware {3D} reconstruction from single and multi-view images.
\newblock In {\em {IEEE/CVF} International Conference on Computer Vision}, pages 2690--2698, 2019.

\bibitem{Wang:2018:Pixel2mesh}
Nanyang Wang, Yinda Zhang, Zhuwen Li, Yanwei Fu, Wei Liu, and Yu{-}Gang Jiang.
\newblock Pixel2mesh: {Generating} {3D} mesh models from single {RGB} images.
\newblock In {\em European Conference on Computer Vision}, volume 11215, pages 55--71, 2018.

\bibitem{Mescheder:2019:Occupancy}
Lars~M. Mescheder, Michael Oechsle, Michael Niemeyer, Sebastian Nowozin, and Andreas Geiger.
\newblock Occupancy networks: Learning {3D} reconstruction in function space.
\newblock In {\em {IEEE} Conference on Computer Vision and Pattern Recognition}, pages 4460--4470, 2019.

\bibitem{Park:2019:Deepsdf}
Jeong~Joon Park, Peter Florence, Julian Straub, Richard~A. Newcombe, and Steven Lovegrove.
\newblock {DeepSDF}: Learning continuous signed distance functions for shape representation.
\newblock In {\em {IEEE} Conference on Computer Vision and Pattern Recognition}, pages 165--174, 2019.

\bibitem{Niemeyer:2020:Differentiable}
Michael Niemeyer, Lars~M. Mescheder, Michael Oechsle, and Andreas Geiger.
\newblock Differentiable volumetric rendering: Learning implicit {3D} representations without {3D} supervision.
\newblock In {\em {IEEE} Conference on Computer Vision and Pattern Recognition}, pages 3501--3512, 2020.

\bibitem{Yariv:2021:Volume}
Lior Yariv, Jiatao Gu, Yoni Kasten, and Yaron Lipman.
\newblock Volume rendering of neural implicit surfaces.
\newblock In {\em Advances in Neural Information Processing Systems}, pages 4805--4815, 2021.

\bibitem{xu2022point}
Qiangeng Xu, Zexiang Xu, Julien Philip, Sai Bi, Zhixin Shu, Kalyan Sunkavalli, and Ulrich Neumann.
\newblock Point-NeRF: Point-based neural radiance fields.
\newblock In {\em Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 5438--5448, 2022.

\bibitem{li2022vox}
Hai Li, Xingrui Yang, Hongjia Zhai, Yuqian Liu, Hujun Bao, and Guofeng Zhang.
\newblock Vox-surf: Voxel-based implicit surface representation.
\newblock {\em IEEE Transactions on Visualization and Computer Graphics}, 2022.

\bibitem{Liu:2020:Neural}
Lingjie Liu, Jiatao Gu, Kyaw~Zaw Lin, Tat{-}Seng Chua, and Christian Theobalt.
\newblock Neural sparse voxel fields.
\newblock In {\em Advances in Neural Information Processing Systems}, pages 15651--15663, 2020.

\bibitem{huang20242d}
Binbin Huang, Zehao Yu, Anpei Chen, Andreas Geiger, and Shenghua Gao.
\newblock 2d gaussian splatting for geometrically accurate radiance fields.
\newblock {\em arXiv preprint arXiv:2403.17888}, 2024.

\bibitem{yu2024gaussian}
Zehao Yu, Torsten Sattler, and Andreas Geiger.
\newblock Gaussian opacity fields: Efficient and compact surface reconstruction in unbounded scenes.
\newblock {\em arXiv preprint arXiv:2404.10772}, 2024.

\bibitem{chen2023neusg}
Hanlin Chen, Chen Li, and Gim~Hee Lee.
\newblock Neusg: Neural implicit surface reconstruction with 3d gaussian splatting guidance.
\newblock {\em arXiv preprint arXiv:2312.00846}, 2023.

\bibitem{long2024adaptive}
Xiaoxiao Long, Yuhang Zheng, Yupeng Zheng, Beiwen Tian, Cheng Lin, Lingjie Liu, Hao Zhao, Guyue Zhou, and Wenping Wang.
\newblock Adaptive surface normal constraint for geometric estimation from monocular images.
\newblock {\em arXiv preprint arXiv:2402.05869}, 2024.

\bibitem{qi2018geonet}
Xiaojuan Qi, Renjie Liao, Zhengzhe Liu, Raquel Urtasun, and Jiaya Jia.
\newblock Geonet: Geometric neural network for joint depth and surface normal estimation.
\newblock In {\em Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition}, pages 283--291, 2018.

\bibitem{fu2022geo}
Qiancheng Fu, Qingshan Xu, Yew~Soon Ong, and Wenbing Tao.
\newblock Geo-NeuS: Geometry-consistent neural implicit surfaces learning for multi-view reconstruction.
\newblock {\em Advances in Neural Information Processing Systems}, 35:3403--3416, 2022.

\bibitem{yoo2009fast}
Jae-Chern Yoo and Tae~Hee Han.
\newblock Fast normalized cross-correlation.
\newblock {\em Circuits, systems and signal processing}, 28:819--843, 2009.

\bibitem{matsuki2023gaussian}
Hidenobu Matsuki, Riku Murai, Paul~HJ Kelly, and Andrew~J Davison.
\newblock Gaussian splatting slam.
\newblock {\em arXiv preprint arXiv:2312.06741}, 2023.

\bibitem{zhang2018unreasonable}
Richard Zhang, Phillip Isola, Alexei~A Efros, Eli Shechtman, and Oliver Wang.
\newblock The unreasonable effectiveness of deep features as a perceptual metric.
\newblock In {\em Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 586--595, 2018.

\bibitem{ye2024absgs}
Zongxin Ye, Wenyu Li, Sidun Liu, Peng Qiao, and Yong Dou.
\newblock Absgs: Recovering fine details for 3d gaussian splatting.
\newblock {\em arXiv preprint arXiv:2404.10484}, 2024.

\bibitem{newcombe2011kinectfusion}
Richard~A Newcombe, Shahram Izadi, Otmar Hilliges, David Molyneaux, David Kim, Andrew~J Davison, Pushmeet Kohi, Jamie Shotton, Steve Hodges, and Andrew Fitzgibbon.
\newblock KinectFusion: Real-time dense surface mapping and tracking.
\newblock In {\em 2011 10th IEEE international symposium on mixed and augmented reality}, pages 127--136. Ieee, 2011.

\bibitem{lorensen1998marching}
William~E Lorensen and Harvey~E Cline.
\newblock Marching cubes: A high resolution 3d surface construction algorithm.
\newblock In {\em Seminal graphics: pioneering efforts that shaped the field}, pages 347--353. 1998.

\bibitem{hedman2018deep}
Peter Hedman, Julien Philip, True Price, Jan-Michael Frahm, George Drettakis, and Gabriel Brostow.
\newblock Deep blending for free-viewpoint image-based rendering.
\newblock {\em ACM Transactions on Graphics (ToG)}, 37(6):1--15, 2018.

\bibitem{cheng2024gaussianpro}
Kai Cheng, Xiaoxiao Long, Kaizhi Yang, Yao Yao, Wei Yin, Yuexin Ma, Wenping Wang, and Xuejin Chen.
\newblock Gaussianpro: 3d gaussian splatting with progressive propagation.
\newblock {\em arXiv preprint arXiv:2402.14650}, 2024.

\bibitem{lu2023scaffold}
Tao Lu, Mulin Yu, Linning Xu, Yuanbo Xiangli, Limin Wang, Dahua Lin, and Bo~Dai.
\newblock Scaffold-GS: Structured 3d Gaussians for view-adaptive rendering.
\newblock {\em arXiv preprint arXiv:2312.00109}, 2023.

%%%%%%%%%%%%%%%%

% \bibitem{kato2018neural}
% Hiroharu Kato, Yoshitaka Ushiku, and Tatsuya Harada.
% \newblock Neural 3d mesh renderer.
% \newblock In {\em Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 3907--3916, 2018.

% \bibitem{keetha2023splatam}
% Nikhil Keetha, Jay Karhade, Krishna~Murthy Jatavallabhula, Gengshan Yang, Sebastian Scherer, Deva Ramanan, and Jonathon Luiten.
% \newblock Splatam: Splat, track \& map 3d gaussians for dense rgb-d slam.
% \newblock {\em arXiv preprint arXiv:2312.02126}, 2023.

% \bibitem{liu2019soft}
% Shichen Liu, Tianye Li, Weikai Chen, and Hao Li.
% \newblock Soft rasterizer: A differentiable renderer for image-based 3d reasoning.
% \newblock In {\em Proceedings of the IEEE/CVF international conference on computer vision}, pages 7708--7717, 2019.


% \bibitem{Sun2022Neural}
% Jiaming Sun, Xi~Chen, Qianqian Wang, Zhengqi Li, Hadar Averbuch{-}Elor, Xiaowei Zhou, and Noah Snavely.
% \newblock Neural 3d reconstruction in the wild.
% \newblock In {\em Special Interest Group on Computer Graphics and Interactive Techniques Conference}, pages 26:1--26:9, 2022.

% \bibitem{yan2023gs}
% Chi Yan, Delin Qu, Dong Wang, Dan Xu, Zhigang Wang, Bin Zhao, and Xuelong Li.
% \newblock Gs-slam: Dense visual slam with 3d gaussian splatting.
% \newblock {\em arXiv preprint arXiv:2311.11700}, 2023.

% \bibitem{zhang2023vis}
% Jingyang Zhang, Shiwei Li, Zixin Luo, Tian Fang, and Yao Yao.
% \newblock Vis-mvsnet: Visibility-aware multi-view stereo network.
% \newblock {\em International Journal of Computer Vision}, 131(1):199--214, 2023.

\end{thebibliography}

==> tables/ablations.tex <==
\begin{table}%[tb]
  \captionsetup{font={footnotesize}}
  \caption{\textbf{Ablation study on the Meetingroom of TnT dataset.}}
  \label{tab:ablation}
  \scriptsize%
  \centering%
  \setlength{\tabcolsep}{5pt}
  \scalebox{1.1}[1.1]{
  \begin{tabu}{c|ccc}
  \toprule
     Model setting & F1-Score$\uparrow$ & PSNR$\uparrow$ \\
  \midrule
  w/o Single-View & 0.26 & 27.76  \\
  w/o Multi-View & 0.15 & 28.43  \\
  w/o Multi-View Geom & 0.23 & 28.34  \\
  w/o Multi-View RGB & 0.20 & 27.62  \\
  w/o Our unbiased depth & 0.20 & 27.10  \\
  %w/o Prune & 0.29 & 27.75 & 2600k \\
  \midrule
  Full model & 0.29 & 27.60 \\
  \bottomrule
  \end{tabu}
  }
  \vspace{-0.3cm}
\end{table}


==> tables/dtu.tex <==
\setlength\tabcolsep{0.5em}
\begin{table*}[tb]
\captionsetup{font={footnotesize}}
\caption{\textbf{Quantitative results of chamfer distance(mm)$\downarrow$ on DTU dataset\cite{jensen2014large}.} PGSR achieves the highest reconstruction accuracy and is over 100 times faster than the SDF method based on NeRF.} 
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccccccclc|c}
\toprule
 \multicolumn{3}{c}{} & 24 & 37 & 40 & 55 & 63 & 65 & 69 & 83 & 97 & 105 & 106 & 110 & 114 & 118 & 122 & & Mean & Time \\ \midrule
 % & NeRF\cite{mildenhall2021nerf} & & 1.90 & 1.60 & 1.85 & 0.58 & 2.28 & 1.27 & 1.47 & 1.67 & 2.05 & 1.07 & 0.88 & 2.53 & 1.06 & 1.15 & 0.96 & & 1.49 & > 12h \\
 % & MVSDF\cite{zhang2021learning} & 0.83 & 1.76 & 0.88 & 0.44 & 1.11 & 0.90 & 0.75 & 1.26 & 1.02 & 1.35 & 0.87 & 0.84 & 0.34 & 0.47 & 0.47 & 0.89 \\
 & VolSDF\cite{Yariv:2021:Volume} & & 1.14 & 1.26 & 0.81 & 0.49 & 1.25 & 0.70 & 0.72 & 1.29 & 1.18 & 0.70 & 0.66 & 1.08 & 0.42 & 0.61 & 0.55 & & 0.86 & \texttt{>} 12h\\
 & NeuS\cite{wang2021neus} & & 1.00 & 1.37 & 0.93 & 0.43 & 1.10 & \tbest 0.65 &  0.57 & 1.48 & 1.09 & 0.83 & 0.52 & 1.20 & 0.35 & 0.49 & 0.54 & & 0.84 & \texttt{>} 12h\\
 %& NeuralWarp\cite{grabocka2018neuralwarp} & & 0.49 & \tbest 0.71 &  0.38 & \tbest 0.38 & \tbest 0.79 & 0.81 & 0.82 & \tbest 1.20 & 1.06 & \tbest 0.68 & 0.66 & \tbest 0.74 & 0.41 & 0.63 & 0.51 & & 0.68 & \texttt{>} 12h\\
 & Neuralangelo\cite{li2023neuralangelo} & & \tbest 0.37 & \tbest0.72 & \tbest 0.35 & \tbest 0.35 & \tbest 0.87 & \best 0.54 & \sbest 0.53 & 1.29 & \tbest 0.97 & 0.73 & \sbest 0.47 & \tbest 0.74 & \tbest 0.32 & \tbest 0.41 &  \tbest 0.43 & & \tbest 0.61 & \texttt{>} 128h\\ \midrule
 & SuGaR\cite{guedon2023sugar} && 1.47 & 1.33 & 1.13 & 0.61 & 2.25 & 1.71 & 1.15 & 1.63 & 1.62 & 1.07 & 0.79 & 2.45 & 0.98 & 0.88 & 0.79 & & 1.33 & 1h\\
 & 2DGS\cite{huang20242d} && 0.48 & 0.91 & 0.39 & 0.39 & 1.01 & 0.83 & 0.81 & 1.36 & 1.27 & 0.76 & 0.70 & 1.40 & 0.40 & 0.76 & 0.52 & & 0.80 & \best 0.32h\\
  & GOF~\cite{yu2024gaussian} & &  0.50 & 0.82 &  0.37 &  0.37 & 1.12 &  0.74 & 0.73 &  \tbest 1.18 & 1.29 & \tbest 0.68 & 0.77 &  0.90 & 0.42 & 0.66 &  0.49 &&  0.74 & 2h\\
 & PGSR(DS) && \sbest 0.34 & \sbest 0.58 & \sbest 0.29 & \sbest 0.29 & \sbest 0.78 & \sbest 0.58 & \tbest 0.54 & \sbest 1.01 & \sbest 0.73 & \sbest 0.51 & \tbest 0.49 & \sbest 0.69 & \sbest 0.31 & \sbest 0.37 & \sbest 0.38 & & \sbest 0.53 & \sbest 0.6h\\
  & PGSR && \best 0.31 & \best 0.52 & \best 0.27 & \best 0.27 & \best 0.76 & \best 0.54 & \best 0.49 & \best 0.98 & \best 0.69 & \best 0.49 & \best 0.46 & \best 0.56 & \best 0.28 & \best 0.35 & \best 0.36 & & \best 0.49 & \tbest 1.0h\\
 \bottomrule
\end{tabular}
}
\label{tab:dtu_result}
\vspace{-0.3cm}
\end{table*}

==> tables/exposure.tex <==
\begin{table}%[tb]
\vspace{-0.2cm}
\captionsetup{font={footnotesize}}
  \caption{\textbf{Ablation study on exposure Compensation.}}
  \label{tab:ablation_exposure}
  \scriptsize%
	\centering%
  \setlength{\tabcolsep}{5pt}
  \scalebox{1.1}[1.1]{
  \begin{tabu}{c|ccc}
  \toprule
     Model setting & F1-Score$\uparrow$ & PSNR$\uparrow$\\
  \midrule
  w/o exposure modeling & 0.76 & 21.71   \\
  w exposure modeling & 0.80 & 25.77  \\
  \bottomrule
  \end{tabu}%
  }
  \vspace{-0.2cm}
\end{table}


==> tables/tnt.tex <==
\begin{table}[t]
\centering
\captionsetup{font={footnotesize}}
\caption{\textbf{Quantitative results of F1 Score$\uparrow$ for reconstruction on Tanks and Temples dataset.} PGSR achieves similar reconstruction accuracy to Neuralgangelo, but our training speed is over a hundred times faster.}
% \vspace{-0.2cm}
\resizebox{0.98\columnwidth}{!}{
\begin{tabular}{@{}l|ccc|ccccc}
% & \multicolumn{3}{c@{}|}{Implicit} & \multicolumn{3}{c@{}}{Explicit} \\ \hline
 & NeuS & Geo-Neus & Neurlangelo & SuGaR & 2D GS & GOF & PGSR\\ 
 \hline
Barn & 0.29 &  0.33 &  \best 0.70  & 0.14 & 0.36 & \tbest 0.51 &  \sbest 0.66\\
Caterpillar & \tbest 0.29 & 0.26 &  \sbest 0.36 & 0.16 & 0.23 & \best 0.41 & \best 0.41\\
Courthouse &  \tbest 0.17 & 0.12 &  \best 0.28 & 0.08 & 0.13 & \best 0.28 & \sbest 0.21\\
Ignatius & \sbest 0.83 & 0.72 &  \best 0.89 & 0.33 & 0.44 & 0.68 & \tbest 0.80\\
Meetingroom & 0.24 & 0.20 &  \best 0.32 &  0.15 & 0.16 & \tbest 0.28& \sbest 0.29\\
Truck &  0.45 & 0.45 &  \tbest 0.48 &  0.26 & 0.26 & \sbest 0.58& \best 0.60\\ 
\hline
Mean & \tbest 0.38 & 0.35 &  \best 0.50 & 0.19 & 0.30 & \tbest 0.46& \best 0.50\\
Time & \texttt{>}24h & \texttt{>}24h & \texttt{>}128h & \tbest 2h & \best 0.57h & \tbest 2h& \sbest 1.2h\\ 
\end{tabular}
}
\label{tab:tnt}
% \vspace{-0.2cm}
\end{table}

% \setlength\tabcolsep{0.5em}
% \begin{table*}[tb]
%   \caption{\textbf{Quantitative results of F1 Score for reconstruction on Tanks and Temples dataset.} PGSR achieves similar reconstruction accuracy to Neuralgangelo, but our training speed is over a hundred times faster.}
%   \label{tab:reconstruction_eval}
%   \scriptsize%
%   \centering%
%   \setlength{\tabcolsep}{5pt}
%   \scalebox{1.1}[1.1]{
%   \begin{tabular}{lccccccc|c}
%   \toprule
%     & Barn & Caterpillar & Courthouse & Ignatius & Meetingroom & Truck & Mean & Time\\
%   \midrule
%   COLMAP\cite{schonberger2016structure} & \tbest 0.55 & 0.01 & 0.11 & 0.22 & 0.19  & 0.19  & 0.21  & - \\
%   Vis-MVSNet\cite{zhang2023vis} & 0.49 & 0.21 & \best0.36 & 0.25 & \best0.43  & 0.28  & 0.34  & -  \\
%   NeuS\cite{wang2021neus} & 0.29 & 0.29 & 0.17 & \sbest0.83  & 0.24  & \tbest0.45  & \tbest0.38  & - \\
%   % NeuS-NGP\cite{chen2023neusg} & 0.46 & \tbest0.32 & 0.08 & 0.81  & 0.08  & 0.44  & 0.37  & 16h \\
%   NeuralWarp\cite{grabocka2018neuralwarp} & 0.22 & 0.18 & 0.08 & 0.02  & 0.08  & 0.35  & 0.15  & - \\
%   Geo-Neus\cite{fu2022geo} & 0.33 & 0.26 & 0.12 & 0.72  & 0.20  & \tbest0.45  & 0.35  & - \\
%   MonoSDF\cite{yu2022monosdf} & 0.49 & 0.31 & 0.12 & \tbest0.78  & 0.23  & 0.42  & \tbest0.39  & 18h \\
%   NeuralAngelo\cite{li2023neuralangelo} & \best0.70 & \sbest0.36 & \sbest0.28 & \best0.89  & \sbest0.32  & \sbest0.48  & \best0.50  & 128h \\ \midrule
%   SuGaR\cite{guedon2023sugar} & 0.04 & 0.03 & 0.01 & 0.07  & 0.04  & 0.08  & 0.05  & 2h \\
%   2DGS\cite{huang20242d} & 0.36 & 0.23 & 0.13 & 0.44  & 0.16  & 0.26  & 0.30  &  0.6h \\
%   PGSR & \sbest0.67 & \best0.41 & \tbest0.22 & \tbest0.80  & \tbest0.29  & \best0.61  & \best0.50  & 1.5h \\
%   \bottomrule
%   \end{tabular}%
%   }
%   \vspace{-0.3cm}
% \end{table*}

